Relativistic Quantum Information: developments in Quantum Information in general relativistic scenarios

Recently, there has been increased interest in understanding entanglement and quantum communication in black hole spacetimes and in using quantum information techniques to address questions in gravity. Studies on relativistic entanglement show the emergence of conceptually important qualitative differences to a non-relativistic treatment. For instance, entanglement was found to be an observer-dependent property that changes from the perspective of accelerated observers moving in flat spacetime. Relativisitic quantum information theory uses well-known tools coming from quantum information and quantum optics to study quantum effects provoked by gravity to learn information about the spacetime. We can take advantage of our knowledge about quantum correlations and effects produced by the gravitational interaction to set the basis for experimental proposals ultimately aiming at finding corrections due to quantum gravity effects, too mild to be directly observed. This doctoral thesis dissertation summarises most of the research carried out during my PhD on this topic.

==> 0c-resumen.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
{\renewcommand{\thechapter}{}\renewcommand{\chaptername}{}
\addtocounter{chapter}{0}
\chapter*{Abstract}\markboth{\sl ABSTRACT}{\sl ABSTRACT}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\addcontentsline{toc}{chapter}{Abstract}

In spite of the impressive progress that cosmology has experienced in recent years, we are still
missing a consistent explanation of the origin of the Universe and the formation of structures,
which should be deduced entirely from a fundamental theory. General Relativity breaks down in the
very initial instants of the history of the Universe, leading to a cosmological singularity of the
big bang type. In this regime General Relativity cannot be trusted, and the very own predictability
of the laws of physics is lost. One expects instead that the physics of the Early Universe
belongs to the realm of Quantum Gravity, namely, a theory of the gravitational field which
incorporates the quantum behavior of nature. One of the most promising candidates for such a theory
is Loop Quantum Gravity. At present, important efforts are being made in order to adapt the
techniques of Loop Quantum Gravity to much simpler settings than those of the complete theory, which
on the other hand remains to be concluded. This is the case of a series of homogeneous cosmological
models obtained from General Relativity by symmetry reduction. The resulting field of research is
known under the general name of Loop Quantum Cosmology (LQC).

As a necessary step towards the extraction of realistic results from LQC, we should consider the
inclusion of inhomogeneities, which play a central role in current cosmology. The main goal of this
thesis is to progress in this direction. With this aim we have studied one of the simplest
inhomogeneous cosmological models, namely the linearly polarized Gowdy $T^3$ model. This model is a
natural test bed to incorporate inhomogeneities in LQC. On the one hand, its quantization by means
of standard techniques has been discussed in detail, and a successful Fock quantization has
already been achieved. On the other hand the subset of its homogeneous solutions describes the
Bianchi I model in vacuo with three-torus topology, and the Bianchi I model has been already
considered within LQC.

We have attained a thorough quantization of this Gowdy model, in which the cosmological singularity
is resolved, by means of a hybrid quantization. This combines the polymeric quantization
characteristic of LQC applied to the homogeneous sector of the (partially reduced) phase space,
which is formed by the set of degrees of freedom that describe the homogeneous Bianchi I
solutions, with a Fock quantization for the inhomogeneities. This approach investigates the effects
of quantum geometry underlying LQC only on the homogeneous sector, while disregards the discreteness
of the geometry encoded by the inhomogeneities. A most natural treatment for the inhomogeneities is
then the Fock quantization. Indeed, one would expect that a quantum field theory for the
inhomogeneities, which can be regarded as a field living on a homogeneous (Bianchi~I) background, be
approximately valid on the polymerically quantized background. 

In order to carry out the loop quantization of the homogeneous sector in the Gowdy model as
rigorously
as possible, we have needed to revisit the very foundations of LQC. We have first reviewed the flat,
homogeneous, and isotropic Friedmann-Robertson-Walker (FRW) universe with a massless scalar field,
which is
a paradigmatic model in LQC. In spite of the prominent role that the model has played in the
development of LQC, there still remained some aspects of its quantization which deserved a more
detailed discussion. These aspects included the kinematical resolution of the cosmological
singularity, the precise relation between the solutions of the densitized and non-densitized
versions of the quantum Hamiltonian constraint, the possibility of identifying superselection
sectors which are as simple as possible, and a clear comprehension of the Wheeler-DeWitt (WDW) limit
associated with
the theory in those sectors. We have revised its quantization by proposing an alternative
prescription when representing the Hamiltonian constraint. Our proposal leads to a
symmetric Hamiltonian constraint operator, which is specially suitable to deal
with all these issues in a detailed and satisfactory way. In particular, with our constraint
operator, the singularity decouples in the kinematical Hilbert space and can be removed already at
this level. Thanks to this fact, we can densitize the quantum Hamiltonian constraint in a
well-controlled manner. Besides, together with the physical observables, this constraint
superselects simple sectors for the universe volume, with a discrete support contained in a single
semiaxis of the real line and for which the basic functions that encode the information about the
geometry possess optimal physical properties: They provide a no-boundary description around
the cosmological singularity and admit a well-defined WDW limit in terms of standing waves.
Both properties explain the presence of a generic quantum bounce replacing the classical singularity
at a fundamental level, in contrast with previous studies where the bounce was proved in concrete
regimes.

Following our program to quantize the Gowdy $T^3$ model, and since the homogeneous sector of this
system coincides with the Bianchi~I model in vacuo with spatial sections of three-torus topology, we
have also faced the quantization of these anisotropic cosmologies in LQC. The implementation of the
so-called \emph{improved dynamics} prescription, which was successfully established for isotropic
situations, gives rise to two different schemes in the presence of anisotropies. The original and
simplest one is a naive adaptation of the isotropic scheme employed for FRW. In turn, the most
recently proposed scheme leads to a more complicated quantum theory. We have investigated the loop
quantization of the Bianchi I model within both
schemes. When representing the Hamiltonian constraint operator, we have followed the same kind of
prescription as in the isotropic FRW model. As a consequence, once again the Hamiltonian constraint
operator leaves suitable subspaces of the kinematical Hilbert space invariant, whose
supports are each contained in a single octant of $\mathbb{R}^3$. This has allowed us to
complete the quantization within both schemes, providing the corresponding physical Hilbert space
and a complete set of physical observables. In both cases, the physical Hilbert space is
superselected in separable sectors. We have analyzed the structure of the resulting superselection
sectors, being those of the second scheme richer and more interesting.

On the other hand, in the vacuum Bianchi I model, and for the simplest scheme of the improved
dynamics, we have explicitly determined the form of the physical solutions to the Hamiltonian
constraint in
terms of elements of the kinematical Hilbert space used to carry out the quantization. This
knowledge makes this model a most appropriate arena to investigate the concept of physical
evolution in LQC in the absence of the massless scalar field which has been used so far in the
literature as an internal time. In order to retrieve the system dynamics when no such a suitable
clock field is present, we have explored different constructions of families of unitarily related
partial observables. These observables are essentially parameterized, respectively, by: $(i)$ one of
the components of the densitized triad, and $(ii)$ its conjugate momentum; each of them
playing the role of an evolution parameter. In order to describe the construction in a simpler
setting, and also for comparison, we have first carried out the analysis in the WDW
quantization of the model, and shown that singularities persist in this quantum approach. In the
loop quantized model the construction is more involved owing to the polymeric nature of the
geometry. Exploiting the properties of the considered example, we have investigated in detail the
domains of applicability of each construction. In both cases the observables possess a neat physical
interpretation only in an approximate sense. However, whereas in case $(i)$ such interpretation is
reasonably  accurate only for a portion of the evolution of the universe, in case $(ii)$ it remains
so during all the evolution (at least in the physically interesting cases). The constructed families
of observables have been next used to describe the evolution of the Bianchi I universe. The
performed
analysis confirms the robustness of the bounces, also in absence of matter fields, as well as the
preservation of the semiclassicality through them. The concept of evolution studied here and the
presented construction of observables are applicable to a wide class of models in LQC, including
the quantization of the Bianchi I model obtained with the other scheme for the improved
dynamics.

Finally, we have implemented the loop quantization of the Bianchi I model corresponding to
each of the two schemes for the improved dynamics in the representation of the homogeneous sector
of the hybrid Gowdy model. For both schemes, the resulting Hamiltonian constraint preserves the
sectors superselected in the Bianchi I model. Thanks to the nice features of these superselection
sectors, we have been able to complete the quantization also in this inhomogeneous system, even
though the homogeneous and inhomogeneous sectors are coupled in a non-trivial way, and now we are
dealing with an infinite number of degrees of freedom. The polymeric quantization of the homogeneous
sector suffices to cure quantum-mechanically the cosmological singularity.
The resulting physical Hilbert space has the
tensor product structure of the physical Hilbert space of the Bianchi I model times a Fock space
which is
unitarily equivalent to the physical space of the conventional Fock quantization of the
deparametrized system. Therefore, we indeed recover the standard quantum field theory for the
inhomogeneities.

In conclusion, we have studied a series of models in the framework of LQC with increasing
complexity, provided by the inclusion of anisotropies and inhomogeneities. We have been able
to improve the LQC techniques that were already developed in homogeneous settings and
complete the quantization of inhomogeneous cosmologies for the first time in the context of LQC.
\cleardoublepage

==> A1-conclusiones.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
{\renewcommand{\thechapter}{}\renewcommand{\chaptername}{}
\addtocounter{chapter}{0}
\chapter*{Conclusiones}\markboth{\sl CONCLUSIONES}{\sl CONCLUSIONES}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\addcontentsline{toc}{part}{Conclusiones}

La motivación principal de esta tesis es extender la aplicabilidad de la cosmología
cuántica de lazos
a situaciones con complejidad suficiente como para permitir la extracción de predicciones físicas
realistas. Con el fin de progresar en esta dirección, hemos analizado la cuantización de diversos
modelos con un orden jerárquico de complejidad, proporcionado por la inclusión de anisotropías e
inhomogeneidades.

\section*{Resultados específicos}

\begin{list}{\labelitemi}{\leftmargin=1em}
 \item Hemos propuesto una nueva prescripción de simetrización y de densitización para el operador
ligadura hamiltoniana, tal que en todos los modelos estudiados:
\begin{itemize}
\item[(i)] El operador resultante desacopla los estados de volumen (homogéneo) nulo. Gracias a
ello, el problema de la singularidad cosmológica inicial queda resuelto cuánticamente incluso sin
restringirse a estados físicos.
\item[(ii)] Dicho operador deja invariantes espacios de Hilbert simples, que son generados
por autoestados de las componentes (homogéneas) de la tríada densitizada, cada una de ellas con una
orientación fija. Como consecuencia, los estados que contienen la información acerca de la
discretización de la geometría verifican una descripción de tipo {ausencia de frontera}, ya
que surgen en una sola sección de volumen (homogéneo) mínimo no nulo. Dichos espacios de
Hilbert proporcionan sectores de superselección que a su vez son simples y tienen propiedades
físicas óptimas.
\end{itemize}
\item En el modelo de FRW acoplado a un campo escalar sin masa, hemos demostrado que los estados
que encierran la información sobre la geometría cuántica convergen a una onda estacionaria
\emph{exacta} en el límite de volumen grande. Este comportamiento, junto con la descripción de tipo
{ausencia de frontera}, muestra la existencia de un rebote cuántico genérico
que reemplaza dinámicamente la singularidad clásica. Por tanto, en este contexto, hemos
demostrado que el mecanismo de resolución de singularidades
mediante un rebote cuántico es una consecuencia directa de los efectos discretos de la geometría que
subyacen en cosmología cuántica de lazos y, por consiguiente, que es una propiedad fundamental de la
teoría.
\item En el modelo de Bianchi I en vacío y en el denominado esquema A para la dinámica mejorada
(esquema factorizable),
el estudio se reduce esencialmente a considerar tres copias del sector gravitacional del modelo de
FRW. Como
consecuencia, los estados que codifican aquí la información sobre la geometría cuántica poseen el
mismo tipo de comportamiento que los análogos del modelo de FRW: descripción de tipo {ausencia
de frontera} y límite de WDW de tipo onda estacionaria. Por tanto, una vez más, existen
rebotes cuánticos genéricos que curan las singularidades.
\item En el modelo de Bianchi I en vacío y en el esquema B (no factorizable), hemos demostrado que
no solo el volumen
toma valores en conjuntos discretos, sino también las variables que representan las anisotropías.
Éstas, sin embargo, no poseen realmente un mínimo, aunque sí un ínfimo nulo. Más aún, en nuestro
análisis,
restringido al sector en el que los autovalores de los operadores
que representan todas las componentes de la tríada densitizada son estrictamente positivos, el
rango de valores de las anisotropías cubre densamente la semirrecta real positiva.
\item Para este modelo, hemos argumentado que los datos iniciales de la sección de volumen mínimo
(no nulo) determinan completamente las soluciones de la ligadura hamiltoniana, y hemos
caracterizado el espacio de Hilbert físico como el espacio de Hilbert de los datos iniciales, cuya
estructura, a su vez, ha sido determinada imponiendo
condiciones de realidad en un conjunto (super) completo de observables físicos.
\item Usando el modelo de Bianchi I en vacío como ejemplo, hemos sido pioneros en analizar y
desarrollar metodológicamente la imagen de evolución física en cosmología cuántica de lazos usando
como tiempo interno alguno de los grados de libertad de la geometría. En particular, hemos llevado a
cabo dos construcciones distintas de observables relacionales o completos, en las que la variable
del espacio de fases que desempeña la función de tiempo interno es, respectivamente: $(i)$ un
parámetro afin asociado a uno de los coeficientes de la tríada densitizada, $(ii)$ su momento
canónicamente conjugado.
\item En ambas construcciones, hemos llevado a cabo un análisis numérico de los valores esperados y
de las dispersiones de los observables, evaluados en estados semiclásicos con perfil gaussiano, que
revela las siguientes predicciones:
\begin{itemize}
 \item[(a)] Los estados gaussianos permanecen picados a lo largo de toda la evolución, en el sentido
de que las dispersiones de los observables se mantienen acotadas.
\item[(b)] En los regímenes de volumen grande, las trayectorias definidas por los valores esperados
de los observables coinciden con las predichas por la relatividad general.
\item[(c)] A medida que las trayectorias se acercan a la ubicación de la singularidad, la dinámica
cuántica se desvía con respecto a la clásica y aparecen rebotes cuánticos que evitan la
singularidad. 
\item[(d)] Además, el límite de WDW de tipo onda estacionaria de las autofunciones de la
cosmología cuántica de lazos nos ha permitido analizar la región asintótica que el cálculo
numérico no permite explorar. Hemos demostrado que el comportamiento semiclásico de estados físicos
muy generales (no solo correspondientes a perfiles gaussianos) se conserva a través del rebote
cuántico.
\end{itemize}
Por el contrario, el mismo tipo de análisis aplicado a la cuantización de WDW del modelo
muestra que esta teoría no cura las singularidades.
\item En el contexto particular del modelo de Gowdy $T^3$, hemos propuesto un procedimiento híbrido,
que combina las cuantizaciones de lazos y de Fock, para tratar la cuantización de cosmologías
inhomogéneas. La cuantización de lazos del sector homogéneo es suficiente para curar la singularidad
cosmológica inicial incluso en el espacio de Hilbert cinemático.
\item Hemos obtenido un operador ligadura hamiltoniana bien definido en un dominio
denso y que conserva los sectores de superselección obtenidos en el modelo de Bianchi I, que, por
tanto, proporcionan en este sistema el sector homogéneo de espacios de Hilbert separables que
también están superseleccionados.
\item Como en modelos anteriores, la ligadura hamiltoniana da lugar a una ecuación en
diferencias en un parámetro interno discreto que tiene un valor mínimo estrictamente positivo.
Hemos demostrado que las soluciones de la ligadura están unívocamente determinadas por los datos
proporcionados en la sección inicial de tal parámetro. Identificando datos iniciales con soluciones,
hemos podido caracterizar el espacio de Hilbert físico como el espacio de Hilbert de los datos
iniciales, cuyo producto interno queda fijado al imponer condiciones de realidad en un conjunto
adecuado de observables.
\item El espacio de Hilbert físico obtenido es el producto tensorial del espacio de Hilbert físico
del modelo de Bianchi I (el correspondiente a cada esquema, A o B) por un espacio de Fock
unitariamente equivalente al obtenido en la cuantización estándar del modelo deparametrizado.
Por tanto, recuperamos la teoría cuántica de campos estándar para las inhomogeneidades, que pueden
enterderse como grados de libertad que se propagan sobre un fondo de tipo Bianchi I.
\item En definitiva, hemos sido capaces de mejorar las técnicas de la cosmología cuántica de lazos
ya antes desarrolladas en contextos homogéneos y de completar la cuantización de cosmologías
inhomogéneas por primera vez dentro del marco de la teoría de lazos.
\end{list}

 
\cleardoublepage




==> referencias.tex <==
\cleardoublepage\addcontentsline{toc}{chapter}{Bibliografía}
%\chapter*{Referencias}

%============================================================
\begin{thebibliography}{999}
%============================================================
%References
%\newpage
%-------------------------------------------------------------

%referencias introducción

%GR

\bibitem{Eins1} A. Einstein, Die Feldgleichungen der Gravitation (The Field Equations of
Gravitation), Sitzungsber. Preuss. Akad. Wiss. Berlin (Math.Phys.), 844 (1915).

\bibitem{Eins2} A. Einstein, Die Grundlage der
Allgemeinen Relativitätstheorie (The Foundation of the General Theory of Relativity), Annalen der
Physik {\bf49}, 769 (1916).

\bibitem{HawEll} S. W. Hawking y G. F. R. Ellis, {\it The Large Scale Structure of Space-Time}
(Cambridge University Press, Cambridge, Inglaterra, 1973).

\bibitem{carlip} Véase, p. ej., S. Carlip, Quantum gravity: A Progress Report,
Rept. Prog. Phys. {\bf64}, 885 (2001).

%loop quantum gravity general
\bibitem{lqg1} T. Thiemann, {\it{Modern Canonical Quantum General Relativity}} (Cambridge University
Press, Cambridge, Inglaterra, 2007).

\bibitem{lqg2} C. Rovelli, {\it{Quantum Gravity}} (Cambridge University Press, Cambridge,
Inglaterra,
2004).

\bibitem{lqg3} A. Ashtekar y J. Lewandowski, Background Independent Quantum Gravity: A Status
Report, Classical Quantum Gravity {\bf 21}, R53 (2004).

\bibitem{lqg4} H. Sahlmann, Loop Quantum Gravity - A Short Review, \texttt{arXiv:1001.4188}. 

\bibitem{dirac} P. A. M. Dirac, {\it Lectures on Quantum Mechanics} (Belfer
Graduate School of Science, Yeshiva University, Nueva York, 1964).

\bibitem{adm1} R. Arnowitt, S. Deser y  C. W. Misner, The Dynamics of General Relativity,
en {\it Gravitation: An Introduction to Current Research}, editado por L. Witten (Wiley, Nueva
York, 1962).

\bibitem{wald} R. M. Wald, {\it General Relativity} (University of Chicago Press, Chicago, 1984).

\bibitem{kuc-ish1} C. J. Isham y K. V. Kucha\v{r}, Representations of Spacetime Diffeomorphisms. I.
Canonical Parametrized Field Theories, Ann. Phys. {\bf164}, 288 (1985).

\bibitem{kuc-ish2} C. J. Isham y K. V. Kucha\v{r}, Representations of Spacetime Diffeomorphisms. II.
Canonical Geometrodynamics, Ann. Phys. {\bf164}, 316 (1985).
%loop quantum cosmology general
\bibitem{lqc1} M. Bojowald, Loop Quantum Cosmology, Living Rev. Rel. {\bf 11}, 4 (2008).

\bibitem{lqc2a} A. Ashtekar, An Introduction to Loop Quantum Gravity through
Cosmology, Nuovo Cim. {\bf122B}, 135 (2007).

\bibitem{lqc2b} A. Ashtekar, Loop Quantum Cosmology: An Overview,
Gen. Rel. Grav. {\bf41}, 707 (2009).

\bibitem{lqc3} G. A. Mena Marug\'an, A Brief Introduction to Loop Quantum Cosmology, AIP Conf.
Proceedings {\bf 1130}, 89 (2009).

%wdw 
\bibitem{witt} B. S. DeWitt, Quantum Theory of Gravity I. The Canonical Theory, Phys. Rev.
{\bf160}, 1113 (1967).

\bibitem{mis-a} C. W. Misner, Quantum Cosmology I, Phys. Rev. {\bf 186}, 1319 (1969).
\bibitem{mis-b} C. W. Misner, Mixmaster Universe, Phys. Rev. Lett. {\bf22}, 1071 (1969).
\bibitem{mis-c} C. W. Misner, Minisuperspace, in {\it Magic Without Magic: John Archibald Wheeler}
(W. H. Freeman, San Francisco, 1972).

\bibitem{hartle} J. B. Hartle, Quantum Cosmology, en {\it High Energy Physics 1985: Proceedings of
the Yale Summer School}, editado por M. J. Bowick y F. Gursey (World Scientific, Singapur, 1985).

\bibitem{hall} Para una guía de la bibliografía sobre cuantización canónica de minisuperespacios,
véase J. J. Halliwell, A Bibliography of Papers on Quantum Cosmology, Int. J. Mod. Phys. A {\bf5},
2473 (1990).

\bibitem{whe} J. A. Wheeler, Superspace and the Nature of Quantum Geometrodynamics, in {\it Batelle
Rencontres}, editado por C. M. DeWitt y J. A. Wheeler (W. A. Benjamin, Nueva York, 1972).

%lqc pionera bojowald
\bibitem{boj1a} M. Bojowald, Loop Quantum Cosmology I: Kinematics, Classical Quantum Gravity
{\bf17}, 1489 (2000).

\bibitem{boj1b} M. Bojowald, Loop Quantum Cosmology II: Volume Operators, Classical Quantum Gravity
{\bf17}, 1509 (2000).

\bibitem{boj1c} M. Bojowald, Loop Quantum Cosmology III: Wheeler-DeWitt Operators; Classical Quantum
Gravity {\bf18} (2001).

\bibitem{boj1d} M. Bojowald,Loop Quantum Cosmology IV: Discrete Time Evolution; Classical Quantum
Gravity {\bf18}, 1701 (2001). 

\bibitem{boj2} M. Bojowald, Absence of Singularity in Loop Quantum Cosmology,
Phys. Rev. Lett. {\bf86}, 5227 (2001).

%lqc isotropa principal
\bibitem{abl} A. Ashtekar, M. Bojowald y J. Lewandowski,  Mathematical Structure of Loop Quantum
Cosmology, Adv. Theor. Math. Phys. {\bf 7}, 233 (2003).

\bibitem{aps1a} A. Ashtekar, T. Paw{\l}owski y P. Singh, Quantum Nature of the Big Bang, Phys.
Rev. Lett. {\bf 96}, 141301 (2006).

\bibitem{aps1b}  A. Ashtekar, T. Paw{\l}owski y P. Singh, Quantum Nature of the Big Bang: An
Analytical and Numerical
Investigation. I, Phys. Rev. D {\bf 73}, 124038 (2006).

\bibitem{aps3} A. Ashtekar, T. Paw{\l}owski y P. Singh, Quantum Nature of the Big Bang: Improved
Dynamics, Phys. Rev. D {\bf 74}, 84003 (2006).

\bibitem{apsv} A. Ashtekar, T. Paw{\l}owski, P. Singh y K. Vandersloot, Loop Quantum Cosmology of
k=1 FRW Models, Phys. Rev. D {\bf 75}, 024035 (2007).

\bibitem{skl} L. Szulc, W. Kami\'nski y J. Lewandowski, Closed FRW Model in Loop Quantum
Cosmology, Classical Quantum Gravity {\bf 24}, 2621 (2007).

\bibitem{vand} K. Vandersloot, Loop Quantum Cosmology and the k = - 1 RW Model, Phys. Rev. D {\bf
75}, 23523 (2007).

\bibitem{luc} L. Szulc, Open FRW Model in Loop Quantum Cosmology, Classical Quantum Gravity {\bf24},
6191
(2007).

\bibitem{tom} E. Bentivegna y T. Paw{\l}owski,  Anti-deSitter Universe Dynamics in LQC, 
Phys. Rev. D {\bf 77}, 124025 (2008).

\bibitem{tom2} W. Kami\'nski y T. Paw{\l}owski, The LQC Evolution Operator of FRW Universe with
Positive
Cosmological Constant, Phys. Rev. D {\bf81}, 024014 (2010).

\bibitem{victor}
V.~Taveras, Corrections to the Friedmann Equations from LQG for a Universe with a Free Scalar Field,
Phys. Rev. D {\bf 78},064072 (2008).

\bibitem{sv-eff}
P.~Singh y K.~Vandersloot, Semi-classical States, Effective Dynamics and Classical Emergence in
Loop Quantum Cosmology, Phys. Rev. D {\bf 72}, 084004 (2005).

\bibitem{cop1} E. J. Copeland, D. J. Mulryne, N. J. Nunes y M. Shaeri, Super-Inflation in Loop
Quantum Cosmology, Phys. Rev. D {\bf77}, 023510 (2008).


\bibitem{cop2} E. J. Copeland, D. J. Mulryne, N. J. Nunes y M. Shaeri, The Gravitational Wave
Background from Super-Inflation in Loop Quantum Cosmology, Phys. Rev. D {\bf79}, 023508 (2009).


\bibitem{grain1} J.~Grain y A.~Barrau, Cosmological Footprints of Loop Quantum
Gravity, Phys. Rev. Lett. {\bf 102}, 081301 (2009).

\bibitem{grain2} J.~Grain, Loop Quantum Cosmology Corrections on Gravity Waves Produced during
Primordial Inflation, \texttt{arXiv:0911.1625}.


%gowdy principal

\bibitem{kuchar2} K. Kucha\v{r}, Canonical
Quantization of Cylindrical Gravitational Waves, Phys. Rev. D {\bf}4, 955 (1971).

\bibitem{gowdy1} R. H.~Gowdy, {Gravitational Waves in Closed Universes},
Phys. Rev. Lett. \textbf{27}, 826 (1971).

\bibitem{gowdy2} R. H. Gowdy, Vacuum Spacetimes with Two-parameter Spacelike Isometry Groups and
Compact Invariant Hypersurfaces: Topologies and Boundary Conditions, Ann. Phys. {\bf83}, 203 (1974).

\bibitem{mon1} V. Moncrief, Global Properties of Gowdy Spacetimes with $T^3\times R$ Topology, Ann.
Phys. {\bf 132}, 87 (1981).

\bibitem{mon2} V. Moncrief, Infinite-dimensional Family of Vacuum Cosmological Models with Taub-NUT
(Newman-Unti-Tamburino)-Type Extensions, Phys. Rev. D {\bf23}, 312 (1981).

\bibitem{ise} J. Isenberg y V. Moncrief, Asymptotic Behavior of the Gravitational Field and the
Nature of Singularities in Gowdy Spacetimes, Ann. Phys. {\bf 199}, 84 (1990).

\bibitem{men1a}
A. Corichi, J. Cortez y G. A. Mena Marug\'{a}n, Unitary Evolution in Gowdy
Cosmology, Phys. Rev. D {\bf73}, 041502 (2006).

\bibitem{men1b}
A. Corichi, J. Cortez y G. A. Mena Marug\'{a}n, Quantum Gowdy $T^3$ Model: A Unitary Description,
Phys. Rev. D {\bf73}, 084020 (2006).

\bibitem{men2} A. Corichi, J. Cortez, G. A. Mena Marug\'{a}n y J. M. Velhinho, Quantum Gowdy
$T^3$ Model: A Uniqueness Result, Classical Quantum Gravity {\bf23}, 6301 (2006).

\bibitem{men3} J. Cortez, G. A. Mena Marug\'{a}n y J. M. Velhinho, Uniqueness of the Fock
Quantization of the Gowdy $T^3$ Model,  Phys. Rev. D {\bf75}, 084027 (2007).

%bianchi I principal y anisótropos y agujeros negros

\bibitem{boj} M. Bojowald, Homogeneous Loop Quantum Cosmology, Classical Quantum Gravity {\bf 20},
2595 (2003).

\bibitem{chio} D. W. Chiou, Loop Quantum Cosmology in Bianchi Type I Models: Analytical
Investigation, Phys. Rev. D {\bf 75}, 024029 (2007).

\bibitem{awe} A. Ashtekar y E. Wilson-Ewing, Loop Quantum Cosmology of Bianchi Type I Models,
Phys. Rev. D {\bf 79}, 083535 (2009).

\bibitem{bdv} M.~Bojowald, G.~Date y K.~Vandersloot, {Homogeneous
Loop Quantum Cosmology: The Role of the Spin Connection}, Classical
Quantum Gravity \textbf{21}, 1253 (2004).

\bibitem{awe2} A.~Ashtekar y E.~Wilson-Ewing, {Loop Quantum
Cosmology of Bianchi Type II Models}, Phys. Rev. D \textbf{80},
123532 (2009).

\bibitem{bdh} M.~Bojowald, G.~Date y G.~M.~Hossain, {The Bianchi
IX Model in Loop Quantum Cosmology}, Classical
Quantum Gravity \textbf{21}, 3541 (2004).

\bibitem{we} E.~Wilson-Ewing, {Loop Quantum Cosmology of Bianchi Type
IX Models}, \texttt{arXiv:1005.5565}.

\bibitem{boj-bh1} M. Bojowald, Spherically Symmetric Quantum Geometry: States and Basic
Operators, Classical Quantum Gravity {\bf21}, 3733 (2004). 

\bibitem{boj-bh2} M. Bojowald y R. Swiderski, The Volume Operator in Spherically Symmetric Quantum
Geometry, Classical Quantum Gravity {\bf 21}, 4881 (2004).

\bibitem{boj-bh3} M. Bojowald, Nonsingular Black Holes and Degrees of Freedom in Quantum
Gravity, Phys. Rev. Lett. {\bf95}, 061301 (2005).

\bibitem{boj-bh4} A. Ashtekar y M. Bojowald, Black hole evaporation: A paradigm,
Classical Quantum Gravity {\bf22}, 3349 (2005). 

\bibitem{boj-bh5} A. Ashtekar y M. Bojowald, Quantum geometry and the Schwarzschild
singularity, Classical Quantum Gravity {\bf23}, 391 (2006).

\bibitem{boj-bh6} M. Bojowald y R. Swiderski, Spherically Symmetric Quantum Geometry: Hamiltonian
Constraint, Classical Quantum Gravity {\bf 23}, 2129 (2006).

\bibitem{pullin1} M. Campiglia, R. Gambini y J. Pullin, Loop Quantization of Spherically Symmetric
Midi-Superspaces, Classical Quantum Gravity {\bf24}, 3649 (2007).

\bibitem{pullin2} R. Gambini y J. Pullin, Black Holes in Loop Quantum Gravity: the Complete
Space-Time, Phys. Rev. Lett. {\bf101}, 161301 (2008).



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% referencias 01-introLQC

\bibitem{adm2} C. W. Misner, K. S. Thorne y J. A. Wheeler, {\it Gravitation} (W. H. Freeman, San
Francisco, 1973).

\bibitem{lqg0aa}  A. Ashtekar, New Variables for Classical and Quantum Gravity, Phys. Rev. Lett.
{\bf57}, 2244 (1986).

\bibitem{lqg0ab}  A. Ashtekar, New Hamiltonian Formulation of General Relativity,  Phys. Rev. D
{\bf36}, 1587 (1987).

\bibitem{lqg0ba} C. Rovelli y L. Smolin, Knot Theory and Quantum Gravity, Phys. Rev. Lett. {\bf61},
1155 (1988).

\bibitem{lqg0bb} C. Rovelli y L. Smolin, Loop Representation for Quantum General Relativity, Nucl.
Phys. B {\bf331}, 80 (1990).

\bibitem{lqg0c} A. Ashtekar, {\it Lectures on Non-Perturbative Canonical Gravity} (World Scientific,
Singapur, 1991).

\bibitem{spin} G. A. Mena Marug\'{a}n, Reality Conditions for Lorentzian and Euclidean Gravity in
the Ashtekar Formulation, Int. J. Mod. Phys. D {\bf3}, 513 (1994).

\bibitem{bar} J. F. Barbero G.,  Real Ashtekar Variables for Lorentzian Signature Space Times,
Phys. Rev. D {\bf51}, 5507 (1995). 

\bibitem{gior1} G. Immirzi, Quantum Gravity and Regge Calculus, Nucl. Phys. B (Proc. Suppl.)
{\bf 57}, 65 (1997).

\bibitem{gior2} G. Immirzi, Real and Complex Connections for Canonical Gravity, Classical Quantum
Gravity {\bf14}, L177 (1997).


\bibitem{ALmeasure1} A. Ashtekar y C.J. Isham, Representations of the Holonomy Algebras of Gravity
and Non-Abelian Gauge Theories, Classical Quantum Gravity {\bf9}, 1433 (1992).

\bibitem{ALmeasure2} A. Ashtekar y J. Lewandowski, Representation Theory of Analytic Holonomy
$C^*$-algebras, en {\it Knots and Quantum Gravity}, editado por J.C Baez (Oxford University Press,
Oxford, 1994). 

\bibitem{baez} J. C. Baez, Generalized Measures in Gauge Theory, Lett. Math. Phys. {\bf31}, 213
(1994).

\bibitem{ALmeasure3} A. Ashtekar y J. Lewandowski, Projective Techniques and Functional Integration
for Gauge Theories, J. Math. Phys. {\bf36}, 2170 (1995).

\bibitem{fleis} C. Fleischhack, Proof of a Conjecture by Lewandowski and Thiemann, Commun. Math.
Phys. {\bf249}, 331 (2004).

\bibitem{lost1} H. Sahlmann y T. Thiemann, Irreducibility of the Ashtekar-Isham-Lewandowski
Representation, Classical Quantum Gravity {\bf23}, 4453 (2006). 

\bibitem{lost2} J. Lewandowski, A. Okolow, H. Sahlmann y T. Thiemann,
Uniqueness of Diffeomorphism Invariant States on Holonomy-flux Algebras,
Commun. Math. Phys. {\bf267}, 703 (2006).

\bibitem{Vel} J. M. Velhinho, The Quantum Configuration Space of Loop Quantum Cosmology, Classical
Quantum Gravity \textbf{24}, 3745 (2007).

\bibitem{SvN1} M. H. Stone,  Linear Transformations in Hilbert Space, III:
Operational Methods and Group Theory, Proc. Nat. Acad. Sci. U.S.A. {\bf16}, 172
(1930).

\bibitem{SvN2} J. von Neumann, Die Eindeutigkeit der Schr\"odingerschen
Operatoren (The Uniqueness of the Schr\"odinger Operators), Math. Ann. {\bf104}, 570 (1931).

\bibitem{area1} C. Rovelli y L. Smolin, Discreteness of Area and Volume in Quantum Gravity, Nucl.
phys. B {\bf442}, 593 (1995); Erratum, Nucl. Phys. B {\bf456}, 753 (1995).

\bibitem{area2} A. Ashtekar y J. Lewandowski, Quantum Theory of Geometry. 1: Area Operators,
Classical Quantum Gravity {\bf14}, A55 (1997).

\bibitem{cs} A. Corichi y P. Singh, Is Loop Quantization in Cosmology Unique?, Phys. Rev.
D {\bf 78}, 024034 (2008).

\bibitem{inv-vol-lqg1} T. Thiemann, Anomaly-Free Formulation of Non-Perturbative Four-Dimensional
Lorentzian Quantum Gravity, Phys. Lett. {\bf B380}, 257 (1996).

\bibitem{inv-vol-lqg2} T. Thiemann, Quantum Spin Dynamics (QSD),
Classical Quantum Gravity {\bf15:}, 839 (1998).

\bibitem{gave1a} D. Marolf, Refined Algebraic Quantization: Systems with a Single Constraint,
\texttt{arXiv:gr-qc/9508015}.

\bibitem{gave1b} D. Marolf, Quantum Observables and Recollapsing Dynamics,
Classical Quantum Gravity {\bf 12}, 1199 (1995).

\bibitem{gave1c} D. Marolf, Observables and a Hilbert Space for Bianchi IX,
Classical Quantum Gravity {\bf 12}, 1441 (1995).

\bibitem{gave1d} D. Marolf, Almost Ideal Clocks in Quantum Cosmology: A Brief
Derivation of Time, Classical Quantum Gravity {\bf 12}, 2469, (1995).

\bibitem{gave2} A. Ashtekar, J. Lewandowski, D. Marolf, J. Mour\~ao y T. Thiemann, Quantization
of Diffeomorphism Invariant Theories of Connections with Local Degrees of Freedom, J. Math. Phys.
{\bf 36}, 6456 (1995).

\bibitem{kale} W. Kami\'nski y J. Lewandowski, The Flat FRW Model in LQC: The Self-Adjointness,
Classical Quantum Gravity {\bf 25}, 35001 (2008).



%%%%%%%%%%%%%%%%%%%%%5
%%%%%%%%%%%%%%%%%%%%%
%referencias 02-introGowdy

%ondas de Einstein-Rosen

%\bibitem{ERwaves} A. Einstein y N. Rosen, On Gravitational waves, J. Franklin Inst.
%{\bf223}, 43 (1937). 

\bibitem{misner} C. W. Misner, A Minisuperspace Example: The Gowdy $T^3$ Cosmology, Phys. Rev. D
{\bf8}, 3271 (1973)

\bibitem{berger1} B. K. Berger, Quantum Graviton Creation in a Model Universe, Ann. Phys. {\bf83},
458 (1974).

\bibitem{berger2} B. K. Berger, Quantum Cosmology: Exact Solution for the Gowdy $T^3$ Model, Phys.
Rev. D {\bf 11}, 2770 (1975).

\bibitem{berger3} B. K. Berger, Quantum Effects in the Gowdy $T^3$ Cosmology, Ann. Phys. {\bf 156},
155 (1984).

\bibitem{pierri} M. Pierri, Probing Quantum General Relativity through Exactly
Soluble Midi-Superspaces. II: Polarized Gowdy models, Int. J. Mod. Phys. D {\bf11}, 135
(2002).

\bibitem{ccq} A. Corichi, J. Cortez y H. Quevedo, On Unitary Time Evolution in Gowdy $T^3$
Cosmologies, Int. J. Mod. Phys. D {\bf11}, 1451 (2002). 

\bibitem{torre} C. G. Torre, Quantum Dynamics of the Polarized Gowdy $T^3$ Model, Phys. Rev. D
{\bf66}, 084017 (2002).

\bibitem{men0}  J. Cortez y G. A. Mena Marug\'{a}n, Feasibility of a Unitary Quantum Dynamics in
the Gowdy $T^3$ Cosmological Model, Phys. Rev. D {\bf72}, 064020 (2005).

\bibitem{dani1} J. Fernando Barbero G., D. Gómez Vergel, E. J. S. Villaseñor, Evolution
Operators for Linearly Polarized Two-Killing Cosmological Models, Phys. Rev. D {\bf74}, 024003
(2006).

\bibitem{men4} A. Corichi, J. Cortez, G. A. Mena Marug\'{a}n y J. M. Velhinho, Quantum Gowdy $T^3$
Model: Schr\"odinger Representation with Unitary Dynamics, Classical Quantum Gravity {\bf23}, 6301
(2006).

\bibitem{men5} J. Cortez, G. A. Mena Marugán y J. M. Velhinho,
Uniqueness of the Fock Representation of the Gowdy $S^1\times S^2$ and $S^3$ Models,
Classical Quantum Gravity {\bf25}, 105005 (2008).

\bibitem{dani2} J. F. Barbero G., D. Gómez Vergel y E. J. S. Villaseñor, Quantum Unitary Evolution
of Linearly Polarized $S^1\times S^2$ and $S^3$ Gowdy Models Coupled to Massless Scalar Fields,
Classical Quantum Gravity {\bf25}, 085002 (2008).

\bibitem{men6} J. Cortez, G. A. Mena Marugán, R. Serôdio y J. M. Velhinho,
Uniqueness of the Fock Quantization of a Free Scalar Field on $S^1$ with Time Dependent Mass,
Phys. Rev. D {\bf79}, 084040 (2009).

\bibitem{men7} J. Cortez, G. A. Mena Marugán y J. M. Velhinho,
Fock Quantization of a Scalar Field with Time Dependent Mass on the Three-Sphere: Unitarity and
Uniqueness, Phys. Rev. D {\bf81}, 044037 (2010).

\bibitem{men8} J. Cortez, G. A. Mena Marugan, J. Olmedo y J. M. Velhinho,
A Unique Fock Quantization for Fields in Non-Stationary Spacetimes, \texttt{arXiv:1004.5320}.


\bibitem{man} G. A. Mena Marug\'{a}n y M. Montejo, Quantization of Pure Gravitational Plane
Waves, Phys. Rev. D {\bf58}, 104017 (1998).

\bibitem{wald2} R. M. Wald, {\it Quantum Field Theory in Curved Spacetime and Black Hole
Thermodynamics} (University of Chicago Press, Chicago, 1994). 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%referencias 3-FRW

\bibitem{Pol} W. Kami\'nski, J. Lewandowski y T. Paw{\l}owski, Physical Time and other Conceptual
Issues of QG on the Example of LQC, Classical Quantum Gravity {\bf 26},
035012 (2009).


\bibitem{mmo} M. Mart\'{\i}n-Benito, G. A. Mena Marug\'{a}n y J. Olmedo, 
Further Improvements in the Understanding of Isotropic Loop Quantum Cosmology, Phys. Rev. D {\bf
80}, 104015 (2009).

\bibitem{acs}A. Ashtekar, A. Corichi y P. Singh, On the Robustness of Key Features of Loop
Quantum Cosmology, Phys. Rev. D {\bf 77}, 024046 (2008).

\bibitem{chinos} Y. Ding, Y. Ma y J. Yang, Effective Scenario of Loop Quantum Cosmology, Phys. Rev.
Lett {\bf 102} 051301 (2009).

\bibitem{red1} A. D. Rendall, Unique Determination of an Inner Product by Adjointness Relations in
the Algebra of Quantum Observables, Classical Quantum Gravity {\bf 10}, 2261 (1993).

\bibitem{red2} A. D. Rendall, Adjointness Relations as a Criterion for Choosing an Inner Product, 
\texttt{arXiv:gr-qc/9403001}.

\bibitem{kp-posL} W. Kami\'nski y T. Paw{\l}owski, Cosmic Recall and the Scattering
Picture of Loop Quantum Cosmology, Phys. Rev. D. {\bf81}, 084027 (2010).

\bibitem{haw1} S. W. Hawking, The Boundary Conditions of the Universe, Pont. Acad. Sci. Varia
{\bf48}, 563 (1982).

\bibitem{haw2} J. B. Hartle y S. W. Hawking, Wave Function of the Universe, Phys. Rev. D {\bf
28}, 2960 (1983).

\bibitem{haw3} S. W. Hawking, The Quantum State of the Universe, Nucl. Phys. B
{\bf239}, 257 (1984).

\bibitem{cs2} A. Corichi y P. Singh, Quantum Bounce and Cosmic Recall, Phys. Rev. Lett. {\bf
100}, 161302 (2008).


%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%
%referencia 04-Bianchi-kin

\bibitem{bianchi} L. Bianchi, Sugli Spazii a Tre Dimensioni che Ammettono un Gruppo Continuo di
Movimenti (On the Spaces of Three Dimensions that Admit a Continuous Group of Movements), Soc.
Ital. Sci. Mem. di Mat. {\bf11}, 267 (1897).

\bibitem{kramer} D. Kramer, H. Stephani, M. MacCallum y E. Herlt, {\it Exact Solutions of Einstein
Field Equations} (Cambridge University Press, Cambridge, Inglaterra, 1980).

\bibitem{aspu} A. Ashtekar y J. Pullin, Bianchi Cosmologies: A New Description, Ann. Israel
Phys. Soc. {\bf 9}, 65 (1990).

\bibitem{neg2} N. Manojlovi\'c  y A. Mikovic, Canonical Analysis of the Bianchi Models in an
Ashtekar Formulation, Classical Quantum Gravity {\bf10}, 559 (1993).

\bibitem{neg1} N. Manojlovi\'{c} y G. A. Mena Marug\'{a}n, Nonperturbative Canonical Quantization of
Minisuperspace Models: Bianchi types I and II, Phys. Rev. D {\bf 48}, 3704 (1993).


\bibitem{chi1} D. W. Chiou y K. Vandersloot, The Behavior of Non-Linear Anisotropies in Bouncing
Bianchi I Models of Loop Quantum Cosmology, Phys. Rev. D {\bf76}, 084015 (2007).

\bibitem{chi2}
D. W. Chiou, Effective Dynamics, Big Bounces and Scaling Symmetry in Bianchi Type I Loop Quantum
Cosmology, Phys. Rev. D {\bf 76}, 124037 (2007).


\bibitem{mmp} M. Mart\'{\i}n-Benito, G. A. Mena Marug\'{a}n y T. Paw{\l}owski, Loop Quantization of
Vacuum Bianchi I Cosmology, Phys. Rev. D {\bf 78}, 064008 (2008).

\bibitem{luc2} L. Szulc, Loop Quantum Cosmology of Diagonal Bianchi Type I model: Simplifications
and Scaling Problems, Phys. Rev. D {\bf78}, 064035 (2008).

\bibitem{mmw} M. Mart\'{\i}n-Benito, G. A. Mena Marug\'{a}n y E. Wilson-Ewing, Hybrid Quantization:
from Bianchi I to the Gowdy Model, \texttt{arXiv:1006.2369}.

\bibitem{kasner} E. Kasner, Geometrical Theorems on Einstein's Cosmological Equations, Amer. J.
Math. {\bf43}, 217 (1921).

%\bibitem{solutions} D. Kramer, H. Stephani, E. Herlt y M. MacCallum, {\it{Exact solutions of
%Einstein's Field Equations}} (Cambridge University Press, Cambridge, Inglaterra, 1980).

\bibitem{cs3} A. Corichi y P. Singh, A Geometric Perspective on Singularity Resolution and
Uniqueness in Loop Quantum Cosmology, Phys. Rev. D {\bf80},044024 (2009).

\bibitem{Vel2} J. M. Velhinho, Comments on the Kinematical Structure of Loop Quantum Cosmology, 
Classical Quantum Gravity {\bf21}, L109 (2004). 


%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
%Referencias evolution

\bibitem{front} S. W. Hawking y C. J. Hunter, The Gravitational Hamiltonian in the Presence of
Non-Orthogonal Boundaries, Classical Quantum Gravity {\bf13}, 2735 (1996).

\bibitem{rovelli-obs1} C. Rovelli, What is Observable in Classical and Quantum Gravity?, Classical
Quantum Gravity {\bf8}, 297 (1991).

\bibitem{rovelli-obs2} C. Rovelli, Partial Observables, Phys. Rev. D {\bf65}, 124013
(2002).

\bibitem{rovelli-obs3} C. Rovelli, Forget time, \texttt{arXiv:0903.3832}.

\bibitem{bianca-obs1} B. Dittrich, Partial and Complete Observables for Canonical General
Relativity,
Classical Quantum Gravity {\bf23}, 6155 (2006).

\bibitem{bianca-obs2} B. Dittrich, Partial and Complete Observables for Hamiltonian
Constrained Systems, Gen. Relativ. Gravit. {\bf39}, 1891 (2007).

 \bibitem{thiemann-obs} T. Thiemann, Reduced Phase Space Quantization and Dirac Observables,
Classical Quantum Gravity {\bf23}, 1163 (2006).

\bibitem{thiemann-obs2} K. Giesel y T. Thiemann, Algebraic Quantum Gravity (AQG) IV. Reduced Phase
Space Quantisation of Loop Quantum Gravity, \texttt{arXiv:0711.0119}.

\bibitem{david1} D. Brizuela, J. M. Martin-Garcia y G. A. Mena Marug\'an, High-Order
Gauge-Invariant Perturbations of a Spherical Spacetime, Phys. Rev. D {\bf76}, 024004 (2007).

\bibitem{david2} D. Brizuela, J. M. Martin-Garcia y M. Tiglio, A Complete Gauge-Invariant
Formalism for Arbitrary Second-Order Perturbations of a Schwarzschild Black Hole, Phys.
Rev. D {\bf80}, 024021 (2009).

\bibitem{mmp2} M. Mart\'{\i}n-Benito, G. A. Mena Marug\'{a}n y T. Paw{\l}owski, Physical Evolution
in Loop Quantum Cosmology: The Example of Vacuum Bianchi I,
Phys. Rev. D {\bf80}, 084038 (2009).

\bibitem{trap-rule} E. W. Weisstein, Trapezoidal Rule. From MathWorld---A Wolfram Web
Resource. http://mathworld.wolfram.com/TrapezoidalRule.html 

\bibitem{FFT} W. H. Press, B. P Flannery, S. A. Teukolsky y W. T. Vetterling, {\it{Numerical Recipes
in
C: The Art of Scientific Computing}} (Cambridge University Press, Cambridge, Inglaterra, 2007).

%%%%%%%%
%gowdy
\bibitem{gow-let} M. Mart\'{\i}n-Benito, L. J. Garay y G. A. Mena Marug\'{a}n, Hybrid Quantum Gowdy
Cosmology: Combining Loop and Fock Quantizations, Phys. Rev. D \textbf{78}, 083516 (2008).

\bibitem{gow-ijmp} G. A. Mena Marug\'{a}n y M. Mart\'{\i}n-Benito,  Hybrid Quantum Cosmology:
Combining Loop and Fock Quantizations, Int. J. Mod. Phys. A {\bf24}, 2820
(2009).

\bibitem{gow-B} L. J. Garay, M. Mart\'{\i}n-Benito y G. A. Mena Marug\'{a}n, Inhomogeneous Loop
Quantum Cosmology: Hybrid Quantization of the Gowdy Model, \texttt{arXiv:1005.5654}.

\bibitem{guille-gow} G. A. Mena Marug\'{a}n, Canonical Quantization of the Gowdy Model, Phys. Rev. 
D {\bf56}, 908 (1997).

\bibitem{date1} K. Banerjee y G. Date, Loop Quantization of Polarized Gowdy Model on $T^3$:
Classical Theory, Classical Quantum Gravity {\bf25}, 105014 (2008).

\bibitem{date2} K. Banerjee y G. Date, Loop Quantization of Polarized Gowdy Model on $T^3$:
Kinematical States and Constraint Operators, Classical Quantum Gravity {\bf25}, 145004 (2008).

\bibitem{rv} C. Rovelli y F. Vidotto, Stepping out of Homogeneity in
Loop Quantum Cosmology, Classical Quantum Gravity {\bf 25}, 225024 (2008).

\bibitem{bhks} M. Bojowald, G. M. Hossain, M. Kagan y S.~Shankaranarayanan, Anomaly Freedom
in Perturbative Loop Quantum Gravity, Phys. Rev. D {\bf 78}, 063547 (2008).

\bibitem{eff} D. Brizuela, G. A. Mena Marug\'an y T. Paw{\l}owski, Big Bounce and Inhomogeneities,
Classical Quantum Gravity {\bf27}, 052001 (2010).

\bibitem{mpw} G. A. Mena Marug\'an, T. Paw{\l}owski y E. Wilson-Ewing, An Effective Analysis of the
Hybrid Quantization of the Gowdy Model ({\it{en preparación}}).
%resolucion singularidades

%\bibitem{sing1} M. Bojowald, Singularities and quantum gravity,

%\bibitem{sing2} A. Ashtekar, Singularity Resolution in Loop Quantum Cosmology: A Brief Overview,
%J. Phys. Conf. Ser. {\bf189}, 012003 (2009). 

%%%%%%%%%%%%%%%%%%

%apendice operadores

\bibitem{functional1} M. Reed y B. Simon, {\it Methods of Modern Mathematical Physics
I: Functional Analysis} (Academic Press, San Diego, 1980).

\bibitem{functional2} A. Galindo y P. Pascual, {\it {Mecánica
Cuántica I}} (Eudema Universidad, Madrid, 1989); {\it{Quantum
Mechanics I}} (Springer-Verlag, Berlin, 1990).

\bibitem{kato} T. Kato, {\it Perturbation Theory for Linear
Operators} (Springer-Verlag, Berlín, 1980).

\bibitem{functional3} L. Abellanas y A. Galindo, {\it {Espacios de Hilbert}} (Eudema
Universidad, Madrid, 1987).


%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%
%nuestra publicaciones




%============================================================
\end{thebibliography}
%============================================================

